Methods for transverse and longitudinal spin-photon coupling in silicon quantum dots with intrinsic spin-orbit effect

In a full-scale quantum computer with a fault-tolerant architecture, having scalable, long-range interaction between qubits is expected to be a highly valuable resource. One promising method of achieving this is through the light-matter interaction between spins in semiconductors and photons in superconducting cavities. This paper examines the theory of both transverse and longitudinal spin-photon coupling and their applications in the silicon metal-oxide-semiconductor (SiMOS) platform. We propose a method of coupling which uses the intrinsic spin-orbit interaction arising from orbital degeneracies in SiMOS qubits. Using theoretical analysis and experimental data, we show that the strong coupling regime is achievable in the transverse scheme. We also evaluate the feasibility of a longitudinal coupling driven by an AC modulation on the qubit. These coupling methods eschew the requirement for an external micromagnet, enhancing prospects for scalability and integration into a large-scale quantum computer.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
